A Federated Lightweight Authentication Protocol for the Internet of Things

Considering the world's IoT development and market, it is necessary to guarantee the security of the developed IoT applications as well as the privacy of their end users. In this sense, Federated Identity Management (FIdM) systems can be of great help as they improve user authentication and privacy. In this paper, we claim that traditional FIdM are mostly cumbersome and then ill-suited for IoT. As a solution to this problem, we come up with a federated identity authentication protocol exclusively tailored to IoT. Federated Lightweight Authentication of Things (FLAT), our solution, replaces weighty protocols and asymmetric cryptographic primitives used in traditional FIdM by lighter ones. For instance, FLAT synergistically combines symmetric cryptosystems and Implicit Certificates. The results show that FLAT can reduce the data exchange overhead by around 31% when compared to a baseline solution. FLAT's Client is also more efficient than the baseline solution in terms of data transmitted, data received, total data exchange, and computation time. Our results indicate that FLAT runs efficiently even on top of resource-constrained devices like Arduino.

==> back.tex <==

\subsection{Background}
\label{sec:back}


This chapter will introduce some necessary concepts related to FLAT, including the characterization of IoT devices, fundamental concepts in FIdM and some cryptosystems used in the solution.

\subsection{IoT}

Society is experiencing an increasing number of connected devices: smartphones, sensors, and computers can communicate and cooperate to perform certain tasks \citep{atzori2010}. In this sense, IoT is a network of everyday objects with certain capabilities communicating to reach a specific goal \citep{whitmore2015}.

There are numerous possibilities in IoT, including applications in several different domains such as healthcare, transportation, smart cities, smart homes, agriculture and traffic management \citep{gubbi2013}. Undoubtedly, IoT can bring a series of advantages and enhancements to businesses and also increase the comfort and quality of services. The possibilities brought by IoT have caught the attention of the scientific community, hence making IoT a research topic of general interest.

Among several open research topics in IoT, there are privacy, standardization and authentication \citep{atzori2010}. FLAT approaches exactly the authentication issue in IoT, considering the lack of computational resources and the potential mobility of devices, as well as other inherent aspects of IoT that are not present in the traditional Internet.


\subsection{IoT Devices}

%As IoT increasingly is part of our daily lives, the number of devices providing different kinds of applications is also growing significantly, involving areas like intelligent transports, industrial automation, health and smart homes \citep{atzori2010}. 

As the IoT devices contemplate environments with very different needs, these devices also have diverse characteristics, varying in size, type, and computational capabilities.

%Among these equipment,
There are devices that have very low computational and storage capabilities, so protocols and processes executed by these devices must be lightweight. Here, this kind of IoT devices will be referred to as restricted devices. As \strt{iotdevices} shows, devices such as Memsic IRIS\footnote{\url{http://www.aceinna.com//wireless-sensor-networks/index.cfm}}, Arduino Mega 2560\footnote{\url{https://store.arduino.cc/usa/arduino-mega-2560-rev3}} and Arduino Due\footnote{\url{https://store.arduino.cc/usa/arduino-due}} are in this category. 
%Note they have significant memory and storage restrictions: less than 0.1 MB of SRAM and less than 1 MB of flash memory. 

There are also devices that do not have major resource constraints, with flash memory in gigabytes and higher CPU speeds. These IoT devices will be referred here as intermediary devices. Raspberry Pi Zero W\footnote{\url{https://www.raspberrypi.org/products/raspberry-pi-zero-w/}} and BeagleBone Black\footnote{\url{https://beagleboard.org/black}}, shown in \strt{iotdevices}, are in this category, both with 512 MB of SRAM. The flash memory in Raspberry Pi Zero W is variable, but there is support for up to 32 GB, while the BeagleBone Black has a flash memory of 4 GB.  

There are also devices in IoT networks that have superior computational power when compared to the devices shown in \strt{iotdevices}. These devices are equivalent to robust servers and equipment found in the traditional Internet. 


\begin{table}[!ht]
\centering
\caption{Examples of IoT devices.}
\label{tab:iotdevices}
\begin{tabular}{l|l|l|l|l}
\textbf{Class}                             & \textbf{Device}            & \textbf{CPU(GHz)}       & \textbf{SRAM(MB)}      & \textbf{Flash(GB)}             \\ \hline
\multirow{3}{*}{restricted}      & Memsic IRIS            & 8.0 x $10^{-3}$               & 7.8 x $10^{-3}$      & 1.2 x $10^{-4}$             \\ \cline{2-5} 
                                   & Arduino Mega 2560      & 1.6 x $10^{-2}$                & 7.8 x $10^{-3}$      & 2.4 x $10^{-4}$             \\ \cline{2-5} 
                                   & Arduino Due            & 8.4 x $10^{-2}$               & 9.4 x $10^{-2}$     & 4.9 x $10^{-4}$             \\ \hline
\multirow{2}{*}{intermediary} & Raspberry Pi Zero W    & 1.0             & 512.0    & until 32.0  \\ \cline{2-5} 
                                   & BeagleBone Black       & 1.0             & 512.0    & 4.0               
\end{tabular}
\end{table} 

In FLAT, the Client device is a restricted IoT device with a high level of mobility. On the other hand, the SP is represented by an intermediary IoT device. 

%One might think of another secondary possibility where a restricted device would be used also for the SP. In this case, the SP would have mobility restrictions, and a gateway could be used to process the authentication protocol. It is important to note that the use of gateways in IoT environments is not the focus of this work, as it is considered primarily that the SP could also have a mobile behavior and a sufficient computational power to process asymmetric cryptographic primitives. 

In some scenarios, the restricted devices might be connected to the network through gateways, which can take care of more complex network and security operations, as gateways are more powerful devices. It is important to note that this work considers the direct connection of restricted devices to the network, and thus, does not make use of gateways to execute authentication and authorization tasks or to connect to the network.

In the authentication protocol proposed here, the only device considered to have a higher computational power, equivalent to servers in the traditional Internet, is the IdP.  

\subsection{IdM and FIdM}

When it comes to security in IoT, IdM has a fundamental role in protecting the network resources, since it controls the access of user and devices to these resources and manages the entire lifecycle of users' (and devices') digital identities \citep{windley2005}. Digital identity, in turn, is a set of attributes or any other data that together can uniquely identify one entity (user, device, institution), usually proven through the use of credentials \citep{windley2005}.

 According to \citeauthor{nogueira2011b} the main operations of an IdM system are: (i) identification, (ii) authentication, (iii) authorization and (iv) auditing \citep{nogueira2011b}. Identification provides an identity to the system. Authentication, in turn, occurs when the system verifies the identity using the credentials. The process of authorization involves granting privileges to an entity after authentication. Auditing is registering the actions of an entity in the system.

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.25]{img/access}
\caption{IdM main operations.}
\label{fig:access}
\end{figure}

For instance, imagine a user would like to access a technical report provided by a technology company (\strf{access}). This user would present her credentials to the company's system to be identified (step 1, \strf{access}). These credentials will be sent to the authentication process (step 2, \strf{access}), where it will verify if the user is legitimate, i.e., if the user is really whom she claims she is. After the authentication process, the system will check the access privileges of the user (authorization process, step 3, \strf{access}) to grant access to the technical report or not (step 4, \strf{access}). The auditing process takes place registering all the details related to these steps in a log file kept by the system.  



\citeauthor{windley2005} defines the specific steps of authorizing the execution of a requested action in an IdM system (\strf{authsteps}) \citep{windley2005}. The user shows her credentials to a \acrfull{pep} and makes a request to the system (step 1, \strf{authsteps}). Then, the PEP will authenticate the user using her credentials in the authentication server (step 2, \strf{authsteps}). The PEP gives the authenticated credentials to the \acrfull{pdp} (step 3, \strf{authsteps}), that using information about the security policy (step 4, \strf{authsteps}) and the identities (step 5, \strf{authsteps}), decides which access permission the user has in the system. This decision is sent to the PEP, denying or allowing the user's request (step 6, \strf{authsteps}). 

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.3]{img/authsteps}
\caption{Authentication and authorization steps. Adapted from \citep{windley2005}.}
\label{fig:authsteps}
\end{figure}

FLAT focus on the authentication part of the IdM system, defining necessary assumptions and implementing the mechanisms to authenticate restricted devices in IoT. When describing FLAT the term Client will be used to refer to the system user/device.

%, as in this case the ones using the services are devices/users. 
 

%(identity provider, authenticates the users and controls the credentials), the SP (service provider, uses an IdP to authenticate users and provides services).




Traditionally, there are three different models used in IdM systems \citep{cao2010}: isolated, centralized and federated.

In the isolated model, a single server is responsible for providing the service and also for storing identity information \citep{cao2010}. In practice, an SP would not only provide the service requested by the user but also performs authentication and authorization tasks. As all the information is stored in each SP, the user would need different credentials for each SP it would like to access, and thus, this solution does not provide good usability (as the user would have to manage several different credentials) and it is also not storage efficient, as the identity information of the same user will be stored in different SPs. This model is represented in \strf{isolated}.

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.25]{img/isolated}
\caption{Isolated IdM model. Based on \citep{cao2010}.}
\label{fig:isolated}
\end{figure}

The centralized model (\strf{centralized}), on the other hand, delegates to a central IdP the task of storing the identity information of all users from all SPs \citep{cao2010}. Differently from the isolated model, there is a clear definition of different entities for SP and IdP, but the identity information that was stored in each SP in the isolated model, are now all placed in a central server, the IdP. As the number of users grows, this model can present scalability problems, since only one entity is responsible for every single user. This model can also be problematic in the occurrence of a security flaw, as all the identity information is centralized: once the IdP is compromised, all user's information is also compromised. 

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.25]{img/centralized}
\caption{Centralized IdM model. Based on \citep{cao2010}.}
\label{fig:centralized}
\end{figure}


In the federated model (FIdM), the IdPs and SPs are in separate servers, as in the centralized model. However, there is more than one IdP. The federated model enables the use of services from different domains by external users in a transparent way: the user credentials are global identities in the federation and the SPs from different domains are a single global SP \citep{cao2010}. \strf{federated} shows the federated IdM model.

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.25]{img/federated}
\caption{Federated IdM model. Based on \citep{cao2010}.}
\label{fig:federated}
\end{figure}

Considering the need for a solution that takes into account the potential mobility of IoT devices between different domains, FLAT adopts a federated model. According to \citeauthor{maler2008}, FIdM is technologies and processes that allow the distribution of identity information and the delegation of activities related to these identities between different domains \citep{maler2008}. The FIdM model allows a domain to manage the identities of external users transparently \citep{josang2005}. It also makes possible the use of SSO, where a user can authenticate a single time to gain access to several services, avoiding frequent login tasks and remembering different authentication data \citep{maler2008}. However, as it involves different domains, FIdM also imposes challenges related to security and system architecture, such as deployment of secure communication, strong authentication mechanisms, user information management to preserve privacy, management of identifiers and IdP discovery \citep{maler2008}.

%, and thus, each domain should implement consistent secure communication, ensuring the use of new devices and   

%For example, in FIdM is possible to authenticate an external user in a local SP without creating a new identity or registering new credentials. 

In FIdM, the SPs and IdPs exchange authentication and authorization messages, so the users from a local system can access resources of an external system that participates in the federation \citep{chadwick2009a}. The information flow in SSO applications in a FIdM model can have different variants, with two main standards being identified: (i) SP-initiated, where the SP sends an explicit access request to the IdP; and (ii) IdP-initiated, where the IdP typically is an access portal so the user can utilize services from several SPs \citep{maler2008}. In the SP-initiated approach, there is the problem of finding the IdP of the user or the so-called \acrfull{wayf}, that can be solved by a smart client (that knows the correct IdP) or even asking the user to choose from a list of IdPs \citep{maler2008}. IdP-initiated approaches, on the other hand, might be susceptible to \acrfull{csrf} \citep{armando2011}.

FLAT adopts the IdP-initiated approach, as the Client needs to contact its IdP before requesting the service to the SP. This choice was made since the IdP works as a \acrfull{kdc} for the symmetric key used in $Client \leftrightarrow SP$ communication, and thus, needs to previously distribute the key before Client and SP can exchange messages. 

\strf{fidm-trad} shows how a traditional FIdM message flow works. Client will make a service request to SP (step 1, \strf{fidm-trad}). The SP, in turn, will redirect the Client to her IdP (step 2, \strf{fidm-trad}). Then, Client asks for an assertion so she can prove her identity to the SP (step 3, \strf{fidm-trad}). Next, the IdP requests and receives the Client's credentials (steps 4 and 5, \strf{fidm-trad}), and sends the assertion to the Client (step 6, \strf{fidm-trad}). The Client forwards the assertion to the SP (step 7, \strf{fidm-trad}) to get access to the service (step 8, \strf{fidm-trad}).

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.7]{img/fidm-trad}
\caption{Traditional FIdM message flow. Based on \citep{birrell2013}.}
\label{fig:fidm-trad}
\end{figure}

There are well-established standards that define the identity information exchange between different domains \citep{shim2005}. \acrfull{saml}, Shibboleth, OAuth, and OpenID Connect are widely used FIdM solutions.

\subsection{SAML}

SAML\footnote{\url{https://www.oasis-open.org/standards\#samlv2.0}} is an ITU (X.1141) and OASIS standard framework based on \acrfull{xml} created to exchange security information and used to enable SSO and identity federation\footnote{\url{http://docs.oasis-open.org/security/saml/Post2.0/sstc-saml-tech-overview-2.0.html}}. The basic components of SAML are assertions, profiles, bindings and protocols \citep{saml2008}. Assertions are a description of attributes, authentication or authorization of an entity. These assertions are sent in a certain format determined by the SAML protocols, which define how the request and response messages should be sent. SAML bindings establish how the integration between SAML messages and communication protocols will be executed. SAML profiles, in turn, are responsible for deciding how all the other components will be described in order to fit the needs of a specific application.

As a protocol made to provide security, it implements not only a standard way of exchanging authentication and authorization messages but also defines security components that should be present, such as XML-signatures, \acrfull{tls} and \acrfull{http} over \acrfull{ssl}. SAML also makes use of XML-encryption. Regarding privacy, SAML supports the use of pseudonyms, transient identifiers, and assurance levels \citep{saml2008}.   

Like in other FIdM systems, a simple authentication flow using SAML starts with the user trying to access a resource in an SP. The user will then receive a SAML request for authentication that will be passed to its IdP. After the user provides her credentials to the IdP, it will build a SAML response regarding the authentication of the user, which is signed by the IdP. The response is passed to the SP, that checks the information in the response and can provide access or not to the requested resource.

SAML is a highly configurable solution, being able to adapt to different application needs. Although SAML is already a consolidated solution and can be integrated into other frameworks, it requires long XML messages and high computational power, as it uses asymmetric cryptography. Thus, it is not adequate for computationally restricted devices and it is not used in FLAT.

\subsection{Shibboleth}

Shibboleth\footnote{\url{https://www.shibboleth.net/}} is an open source federated SSO solution based on SAML 2.0. There are mainly three components in Shibboleth: the IdP, the SP and the \acrfull{ds}. As in other FIdM solutions, the SP provides services to the users and the IdP is responsible for the identities and authentication. The DS is responsible for finding out which IdP holds the identity information about a specific user\footnote{\url{https://wiki.shibboleth.net/confluence/display/CONCEPT}}. Shibboleth also carries the advantages of FIdM systems already mentioned in this chapter, such as increased user privacy and usability. 

The typical flow in Shibboleth is similar to other FIdM solutions, starting with the user trying to access a service in the SP \citep{shibboleth2018}. After the IdP discovery process, the user will receive an authentication request from the SP and will redirect it to the IdP. Depending on the SAML binding and profile determined by the SP, the authentication response provided by the IdP will contain more or less attributes regarding the identity of the user in the SAML assertion. With this authentication response, the SP can then decide if it will authorize or not the access to the resource. Note that in this context, the IdP is responsible for authentication, while the SP is responsible for authorization. It relies in a previously established trust between the SPs and IdPs in the federation, as in other FIdM solutions.   

As mentioned before, Shibboleth is a solution based on SAML, and thus, also incurs in the costs related to the use of the framework, as explained in the previous subsection. FLAT, on the other hand, does not incorporate SAML and makes use of only symmetric cryptography in the Client side, in order to be a more suitable and lightweight solution for IoT.

%Shibboleth does not define the form of authentication the IdP should perform, letting this decision to the organization deploying the solution. 

\subsection{OAuth}

OAuth\footnote{\url{https://oauth.net/}} is an open authorization framework and an \acrfull{ietf} standard -- \acrfull{rfc} 6749. OAuth aims to be a secure authorization solution for accessing HTTP services/resources \citep{rfc6749}. OAuth provides a layer of secure authorization in order to enable limited access to protected resources through access tokens, that contains access attributes restricting the time and scope of the permission \citep{rfc6749}. Although OAuth is an authorization solution, it is usually integrated into other tools to provide authentication and authorization, enabling the user to log in and enjoy services in third-party websites using her credentials from an existing account. 

The participating entities of an OAuth flow are the resource owner, the resource server, the Client and the authorization server. The resource owner, as the name says, owns a resource that should be protected when being accessed by a Client. The resource is hosted in the resource server. The Client is an entity that would like to access the protected resource. The authorization server, under authorization provided by the resource owner, provides access tokens to the Client, so she can access the resource \citep{rfc6749}.

In a typical scenario, a Client makes an authorization request to the resource owner, that then provides an authorization grant (credential granting resource owner authorization) to the Client. Client forwards the authorization grant to the authorization server, in order to get an access token. With the access token, Client can contact the resource server again and get access to the protected resource \citep{rfc6749}.

OAuth is used with HTTP and TLS and is highly configurable, making it possible to interoperate with other solutions to enable authorization in several different applications. Differently from OAuth, FLAT is an authentication solution, not an authorization framework. 

\subsection{OpenID Connect} 

OpenID Connect\footnote{\url{http://openid.net/connect/}} is a solution built on top of OAuth 2.0, providing an identity layer able to verify identities in the authentication process. OpenID Connect integrates an authentication solution to the authorization defined in OAuth 2.0, using \acrfull{json} Tokens to communicate authentication information \citep{openid2014}. \acrfull{jws} and \acrfull{jwe} are used to protect the integrity and confidentiality of the exchanged messages.

In OpenID Connect basic flow, the Client sends a request to the OpenID Provider (OAuth 2.0 authorization server with authentication capabilities). Using the terms of OAuth, the resource owner will then be authenticated in the OpenID Provider. With the authorization of the resource owner, the OpenID Provider is able to provide an ID Token together with an access token to the Client \citep{openid2014}. This ID token is one of the most important extensions of OpenID to OAuth, since it is responsible to provide information about the authentication of the resource owner, including the intention of the authentication and its expiration. The Client sends the access token to the protected resource, being returned an authorization grant. 
%being returned authorized information about the resource owner.

OpenID Connect also allows the use of levels of assurance and is implemented using a REST-like approach \citep{openid2014}. OpenID, however, is also based on asymmetric cryptography, and thus, not adequate to the IoT environment where restricted devices will also make authentication requests. FLAT only uses symmetric cryptography on the Client side, allowing even resource-constrained devices to run the protocol and authenticate.


% The federated model has the advantages of providing cross domain access, higher user control over her data and avoiding the use of several different credentials for each service the user would like to access. There are now many solutions, protocols and standards in FIdM 

\subsection{Cryptosystems}

This section presents a description of the cryptosystems used in FLAT and the reasons why they were chosen as lightweight alternatives to the IoT context.

\subsection{ECDSA and ECIES}

%Elliptic Curve Cryptography (ECC), proposed by Victor Miller \citep{miller1985} and Neal Koblitz \citep{koblitz1987} refers to cryptosystems whose security is based on the discrete logarithm problem for elliptic curves. This problem does not have a known solution in exponential time, and thus, in these cryptosystems is possible to obtain the same security level with significantly smaller keys, when compared to algorithms based on the discrete logarithm problem for finite sets or even the integer factorization problem \citep{johnson2001}.

The discrete logarithm problem for elliptic curves, in which the \acrfull{ecc} is based, does not have a known solution in subexponential time, and thus, in cryptosystems based on ECC is possible to obtain the same security level with significantly smaller keys, when compared to algorithms based on the discrete logarithm problem for finite sets or even the problem of integer factorization~\citep{johnson2001}. The use of shorter keys provides a set of advantages to ECC-based algorithms such as lower requirements for storage and memory, less bandwidth to transmit keys over the network, and less energy consumption in restricted devices~\citep{martinez2010}. \acrfull{ecies} is an asymmetric encryption algorithm based on ECC, and thus, is able to provide the same security level of traditional algorithms (such as RSA) with the use of smaller keys. For example, considering a security level of 128 bits, using RSA the key length would be around 3072 bits while using ECC the key length can be as short as 256 bits~\citep{martinez2010}. The operation of ECIES is described using three procedures \citep{sec12009}: 

\begin{itemize}
\item key deployment: after defining a set of parameters to be used in the scheme (MAC function, symmetric encryption scheme, elliptic curve parameters, point compression), the entity V (the recipient of the encrypted message) generates an elliptic curve key pair $(d_V,Q_V)$ and ensures that U (the sender of the encrypted message) receives the public key $Q_V$.
\item encryption: to encrypt a message $M$, entity U generates an elliptic curve key pair $(k,R)$, where $R=(x_R,y_R)$. U derives a shared secret $z$ using the secret key $k$ and the public key $Q_V$ generated by $V$. Next, U uses a key derivation function to generate a symmetric key $K$ from $z$. U parses the $a$ leftmost bits to form an encryption key $EK$ and the $b$ rightmost bits to form a MAC key $MK$, where $a$ is the size of the key used in the symmetric encryption scheme chosen and $b$ is the size of the key used in the MAC algorithm chosen. U then uses the key $EK$ to encrypt the message $M$, generating ciphertext $EM$. Finally, U computes the tag $D$ on the ciphertext $EM$ using the MAC scheme and the key $MK$. The final ciphertext output by ECIES is the triple $C=(R,EM,D)$. 
\item decryption: Upon the reception of ciphertext $C$, V first needs to parse $C$ to recover $R$, $EM$ and $D$. V derives a shared secret $z$ using her secret key $d_V$ and the public key $R$. V then uses a key derivation function to obtain the key $K$ from $z$. Next, V parses the $a$ leftmost bits to form an encryption key $EK$ and the $b$ rightmost bits to form a MAC key $MK$, where $a$ is the size of the key used in the symmetric encryption scheme chosen and $b$ is the size of the key used in the MAC algorithm chosen. V uses the MAC algorithm chosen to check the tag $D$ and verify it is the tag on $EM$. The last step in the decryption procedure is to decrypt $EM$ using $EK$ to obtain the original message $M$.    
\end{itemize} 

ECIES is also an \acrshort{ansi} (ANSI X9.63), \acrshort{ieee} (IEEE 1363a), \acrshort{iso} (ISO 18033-2) and \acrshort{secg} (SECG SEC1) standard. The use of smaller keys and its consequent advantages make ECIES a good asymmetric encryption solution to IoT, and thus, was chosen as the asymmetric encryption scheme used in FLAT.

The \acrfull{ecdsa}, as the name indicates, is a digital signature algorithm equivalent to the \acrfull{dsa} but based on ECC. ECDSA provides faster signature generation when compared to DSA, since it is possible to achieve the same security level with smaller parameters. There are three different procedures necessary for the functioning of ECDSA \citep{sec12009}:

\begin{itemize}
\item key deployment: after defining a set of parameters to be used in the scheme (hash function, elliptic curve parameters), entity U (the subject of the signature, who signs) generates an elliptic curve key pair ($d_U$, $Q_U$) and entity V (the recipient of the signature) receives the public key $Q_U$.
\item signing: U generates an elliptic curve key pair ($k$,$R$), where $R=(x_R,y_R)$. U then sets $r=x_R$ and computes the hash $e$ of the message $M$ to be signed: $e = H(M)$. Next, U computes $s=k^{-1}(e+rd_{U})$ $(mod$ $n)$, where $n$ is the order of the base point generator. The signature is the pair $S = (r,s)$. 
\item verifying: to verify the signature of U over $M$, V needs to compute the hash of $M$: $e=H(M)$. Then V computes $u_1$ and $u_2$ using the two parts of the signature ($r$ and $s$): $u_1=es^{-1}$ $mod$ $n$ and $u_2=rs^{-1}$ $mod$ $n$. Next, V computes $R = (x_R,y_R)=u_1G+u_2Q_U$, where $G$ is the base point generator. V then sets $v = x_R$ and compares $v$ and $r$: if $v$ is equal to $r$ the signature is valid.   
\end{itemize} 

Using point compression, ECDSA is able to produce public key certificates around 25\% smaller than other algorithms based on asymmetric cryptography \citep{johnson1998}. ECDSA is an ISO (ISO 14888-3), ANSI (ANSI X9.62), IEEE (IEEE 1363-2000), FIPS (FIPS 186-2) and SECG (SEC 1) standard.

ECDSA is used as the digital signature algorithm in FLAT, given the characteristics and advantages presented by ECC in general and by the ECDSA itself.

%Given the characteristics and advantages presented by ECC in general and by ECDSA, it is used in FLAT as the digital signature algorithm of the authentication solution.


\subsection{ECQV}

The \acrfull{ecqv} certificate~\citep{ecqv2001} is an implicit certificate scheme, where the public key is reconstructed from public data~\citep{ecqv2001}. The public key is not stored explicitly in the certificate, eliminating the need for separate public key and signature fields (as in traditional certificates) and thus, provides a smaller certificate, when compared to traditional solutions such as RSA or ECDSA certificates. For instance, considering a security level of 128 bits, while an implicit certificate size is around 257 bits of length (plus identification data), an ECDSA certificate is around 769 bits and an RSA certificate is around 6144 bits \citep{certicom2018}. 

%while an implicit certificate size is around 264 bits of length (plus identification data), an ECDSA certificate is around 776 bits and an RSA certificate is around 6144 bits \citep{certicom2018}. 

%While an implicit certificate is around 4p bits (where p is the security level), an RSA certificate can have 2-4 KB \citep{simplicio2017}.

The main operations of the implicit certificate scheme (ECQV) are \citep{sec42013}:
  
\begin{itemize}
\item setup: the \acrfull{ca} establishes the elliptic curve domain parameters and the hash function and generates a key pair. Formally, the CA generates an elliptic curve key pair ($d_{CA}$, $Q_{CA}$), where $d_{CA}$ is the private key and $Q_{CA}$ is the public key. $Q_{CA}$ is also distributed to U, the subject requesting a certificate, and to V, the one that will receive the certificate.
\item certificate request: the subject who is requesting a certificate to the CA generates a key pair and sends a certificate request to the CA using its public key. Formally, U generates an elliptic curve key pair ($k_{U}$, $R_{U}$), where $k_{U}$ is a private value necessary to compute the private key, and $R_{U}$ is a public value. U also generates a string $U$, that represents her identity. The pair ($U$, $R_{U}$) is the certificate request that will be sent to the CA.
\item certificate generation: CA generates and sends an implicit certificate to the subject after confirming her identity and receiving the certificate request. Formally, the CA generates an elliptic curve key pair ($k$, $kG$), where the value $k$ is private and the value $kG$ is public. The CA then computes $P_{U} = R_{U} + kG$, an elliptic curve point that is the public key reconstruction data. The certificate $Cert_{U} = (P_{U}$ $|$ $U)$ is the concatenation of the public key reconstruction data and $U$, the value representing the identity of U. Next, the CA computes $e = H(Cert_{U})$ as the hash of the certificate $Cert_{U}$. Finally, the CA computes the private key contribution data $r = ek + d_{CA} (mod$ $n)$, where $n$ is the order of the base point generator.
\item public key extraction: extracts the public key of the subject using CA's public key, the implicit certificate and the elliptic curve domain parameters. When the certificate receiver V receives the certificate, it has to extract the public key. Formally, V computes $e = H(Cert_{U})$ as the hash of the certificate received. Then, V computes $Q_{U} = eP_{U} + Q_{CA}$, using the public key reconstruction data from the certificate and the CA's public key. $Q_{U}$ is U's public key extracted from the certificate.  
\item certificate reception: when the subject receives the certificate, she checks that the implicit certificate she received is valid. Formally, U extracts the public key from the certificate, computing the hash of the certificate $e = H(Cert_{U})$ and then calculating $Q_{U} = eP_{U} + Q_{CA}$ to obtain the public key. Then U computes $d_{U} = r + ek_{U} (mod$ $n)$ to obtain the private key. Next, U computes $Q'_{U} = d_{U}G$, where $G$ is the base point generator. If $Q'_{U}$ is equal to $Q_{U}$, then the certificate is valid.
\end{itemize} 

As explained above, the only operation necessary when the receptor of the certificate (relying party) receives the implicit certificate, is the public key extraction. This makes implicit certificates also more computationally efficient than traditional certificates since the process of extracting the public key is faster than signature verification (of the CA's explicit signature) in traditional certificates \citep{certicom2018}. Differently from traditional certificates, in implicit certificates, after being extracted, the public key will only be validated when it will be used in some communication process, with the same being applied to the proof that the subject of the certificate really has knowledge of the private key \citep{ecqv2001}. This means that the association of the public key to its owner and the ownership of the private key are not distinct processes \citep{ecqv2001}. 

%In explicit certificates, the association of the public key to its owner and possession of the private key are two separate processes \citep{ecqv2001}. 

%Another difference between traditional certificates and implicit certificates is that in implicit certificates, after being extracted, the public key will only be validated when it will be used in some communication process, with the same being applied to the proof that the subject of the certificate really has knowledge of the private key \citep{ecqv2001}. In explicit certificates, upon receiving the certificate the recipient can validate the public key, but the proof that the subject of the certificate knows the private key will only be acquired when the keys will be used in some communication process \citep{ecqv2001}. 

FLAT uses implicit certificates in the communication between SP and IdP, in order to reduce communication, storage, and computational costs.

\subsection{Summary}

In this chapter was presented a characterization of the IoT devices considered in this project as well as existing FIdM technologies and their differences when compared to FLAT. Selected cryptosystems were also described, followed by an explanation of why they were chosen to integrate FLAT. The next chapter will cover previous works related to FLAT.


%FLAT uses ECQV as the certificates being exchanged between the SP and IdP, in order to reduce communication, storage and computational costs.

%Furthermore, the signature verification in the ECQV certificate is not explicit, making ECQV more computationally efficient, when compared to traditional certificates~\citep{brown2001}. 

 









%Nossa proposta, o \gls{tool}, define processos para a autenticação de dispositivos, assumindo que as informações de identidade estão distribuídas nos \gls{idp}s das federações participantes. Para acesso aos serviços, mesmo que de um domínio diferente daquele de origem do dispositivo, é delegada ao seu respectivo \gls{idp} a tarefa de autenticação, entrando em contato com o \gls{sp} assim que recebe o pedido de seu respectivo \Cliente{}. O protocolo \gls{tool}, descreve a troca de mensagens entre as entidades envolvidas, para que ocorra a autenticação do dispositivo. Portanto, \gls{tool} é um modelo de autenticação federado iniciado por \gls{idp}, leve e exclusivamente adaptado para o ambiente \gls{iot}. Em nossa solução, o \Cliente{} utiliza apenas primitivas criptográficas simétricas e certificados de tamanho reduzido, de forma a minimizar custos de comunicação, processamento e armazenamento.





















  








































